Interactive Image Generation Using Scene Graphs

Recent years have witnessed some exciting developments in the domain of generating images from scene-based text descriptions. These approaches have primarily focused on generating images from a static text description and are limited to generating images in a single pass. They are unable to generate an image interactively based on an incrementally additive text description (something that is more intuitive and similar to the way we describe an image). We propose a method to generate an image incrementally based on a sequence of graphs of scene descriptions (scene-graphs). We propose a recurrent network architecture that preserves the image content generated in previous steps and modifies the cumulative image as per the newly provided scene information. Our model utilizes Graph Convolutional Networks (GCN) to cater to variable-sized scene graphs along with Generative Adversarial image translation networks to generate realistic multi-object images without needing any intermediate supervision during training. We experiment with Coco-Stuff dataset which has multi-object images along with annotations describing the visual scene and show that our model significantly outperforms other approaches on the same dataset in generating visually consistent images for incrementally growing scene graphs.

==> Multimodal - ICLR 2019-new-2/conclusion.tex <==
\section{Discussion and Future Work}
In this paper, we proposed an approach to sequentially generate images using incrementally growing scene graphs with context preservation. Through extensive evaluation and qualitative results, we demonstrate that our approach is indeed able to generate an image sequence that is consistent over time and preserves the context in terms of objects generated in previous steps. 
%To the best of our knowledge, this is the first attempt in the direction of incremental image generation using scene composition. 
In future, we plan to explore generating end-to-end with text description by augmenting our methodology with module to generate scene graphs from language input. While scene-graphs provide a very convenient modality to capture image semantics, we would like to explore ways to take natural sentences as inputs to modify the underlying scene graph. The current baseline method does single shot generation by passing the entire layout map through the Cascade Refinement Net for the final image generation. We plan to investigate whether the quality of generation can be improved by instead using attention on the GCN embeddings during generation. This could also potentially make the task of only modifying certain regions in the image easier. Further, we plan to explore better architectures for image generation through layouts for higher resolution image generation.

\section*{Acknowledgements}
We would like to thank Dr. Louis-Philippe Morency and Varun Bharadhwaj Lakshminarasimhan for their guidance and for providing us the opportunity to work on this project through the Advanced Multi-Modal Machine Learning (11-777) course from Language Technologies Institute (LTI) at Carnegie Mellon University.

% We intend to explore the following avenues for improving upon existing methods: 

% \begin{enumerate}


    
%     \item Generation of Scene Graph from the language input: While scene-graphs provide a very convenient modality to capture image semantics, we would like to explore ways to take natural sentences as inputs to modify the underlying scene graph. Some work has been previously done on parsing sentences into scene graphs \cite{schuster2015generating}. However, incrementally modifying this graph based on additional sentences is a harder problem, specially because there are no obvious sources of data for it.
    
%     \item Attention over GCN: Previous works based on text-based image generation have used attention to focus on generation of individual objects. The current baseline method does single shot generation by passing the entire layout map through the Cascade Refinement Net for the final image generation. We plan to investigate whether the quality of generation can be improved by instead using attention on the GCN embeddings during generation. This could also potentially make the task of only modifying certain regions in the image easier.
    
% \end{enumerate}


% Our proposed methods will involve the following research challenges:
% \begin{itemize}
%     \item Preserving language semantics breaking or building up scene graphs.
%     \item Preserving previous context (image global structure and objects) during image generation
%     \item Improvement/Preservation of image quality: Since GANs are based on a generative model that sample inputs from a latent space, a naive GAN-based approach for image generation will fail to preserve the information of the image at the input (or previous generation).
%     \item Objective function for providing intermediate supervision. There are several conceivable losses that can be used in the intermediate steps, and we would have to determine empirically which combination of losses work best.

% \end{itemize}

% \section{Acknowledgement}
% We would like to thank Dr L.P. Morency and the 11-777 TAs for their valuable guidance throughout the project. We also thank Justin Johnson for sharing his implementation of sg2im.

{\small
\bibliographystyle{iclr2019_conference}
\bibliography{iclr2019_conference}
}
% \clearpage
% \section{Appendix}

% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.75\linewidth]{images/attn_results_3.png}
% \end{center}
%   \caption{Results from AttnGAN showing the limitation of the approach in handling lengthy textual descriptions with a lot of objects.}
% \label{fig:attn_results3}
% \end{figure}


% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=\linewidth]{images/sg2im_results_4.png}
% \end{center}
%   \caption{Sample images generated using \cite{johnson2018image} with incrementally growing scene graphs. Clearly the image quality is poor at the expense of preserving the semantics of the image and the consistency between the images is low. Moreover, we can observe that model has a bias toward stuff entities with the generation of object entities being much worse than stuff entities.}
% \label{fig:sg2im_results3}
% \end{figure}



==> Multimodal - ICLR 2019-new-2/experiments.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{images/comparison_2.png}
    \caption{Comparison of our results with baseline approaches--sg2im and AttnGAN. While sg2im captures the scene graph's semantic context, it lacks consistency over multiple passes and the generated images are of poor quality. AttnGAN on the other hand generates higher resolution images but doesn't capture semantic context from the scene graph. Our model addresses both of these shortcomings by incrementally adding objects in accordance with the scene graph and  generating higher quality images.  }
    \label{fig:comparison}
\end{figure*}


\section{Experiments}
\label{experiments}
\subsection{Dataset}
% We focus on the COCO dataset for our experiments. COCO is a large image dataset designed for object detection, segmentation, person keypoints detection, stuff segmentation, and caption generation.

We perform experiments on the 2017 COCO-Stuff
dataset \cite{caesar2016coco} which augments a subset of the COCO dataset \citep{lin2014microsoft} with additional stuff categories. The dataset annotates 40K train and 5K validation images with bounding boxes and segmentation masks for 80 `thing' categories (people, cars, etc.) and 91 `stuff' categories (sky, grass, etc.).




We follow the procedure described in \cite{johnson2018image} to construct synthetic scene graphs from these annotations based on the 2D image coordinates of the objects, using six mutually exclusive geometric relationships: left of, right of, above, below, inside, and surrounding. We create three splits for each image based on the number of objects in it. We randomly select 50\% of the objects for the first split and incrementally add 25\% objects for the next two splits. We then synthetically create separate scene graphs for each split. We train incremental generation for three steps, but this can be easily extended to more number of steps.

% \textcolor{red}{mention again the challenges of using real dataset - no intermediate supervision : \\
Note that previous works like \cite{elkeep} have relied on entirely synthetic datasets. For synthetic datasets, intermediate ground truth for all interim stages of the input text can easily be generated. However, for interactive image generation to be truly useful, it needs to generate realistic looking images not constrained to a synthetic dataset's subspace. The challenge with using real datasets like COCO is that we do not have ``ground-truth'' images corresponding to interim scene graphs (i.e., where all objects of the training image are not present). Only at the final step, with the full scene graph, do we get supervision from the training image. This makes our loss formulation described in the previous section particularly important.
% }

To enable comparison against \cite{johnson2018image}, we follow their dataset preprocessing steps. They ignore objects covering less than 2\% of the image, and use images with 3 to 8 objects. They divide the COCO-Stuff 2017 validation set into their own validation and test sets, which contain 24,972 train, 1024 validation, and 2048 test images. For fair comparison, we do the same.


% \begin{itemize}
%     \item Inception Scores: We aim to evaluate quality of the generated images using Inception scores \cite{salimans2016improved}, which uses an ImageNet based classifier to provide a quantitative evaluation of how realistic generated images appear. The effectiveness of our various proposed methods to improve image quality and prove intermediate supervision can be examined by performing an ablation study using Inception scores.
    
%     \item User Studies: As proposed in \cite{johnson2018image}, a second evaluation of the the generated images can be obtained by asking users to classify whether generated images look real, as well as whether they correctly reflect the modifications in the scene graph.
% \end{itemize}

% Detailed qualitative and quantitative analysis of our results and comparisons against the baseline models follow in the next subsections.

% All the instructions required to replicate our baseline experiments can be found in their respective Github repositories. \footnote {\url{https://github.com/taoxugit/AttnGAN} }
% \footnote{\url{https://github.com/google/sg2im}}

\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/results_collage_4.png}
    \caption{Sample outputs of our pipeline, visualized over 3 steps of generation. 3 splits for each image are created, based on the number of objects in that image. Synthetic scene graphs are then generated for each split and used for incremental image generation. While three steps are used for training, this method is quite easily extensible for more number of steps as well.}
    \label{fig:sample_outputs}
\end{figure*}


\subsection{Qualitative Results}
We compare the performance of our model against two baselines \citep{johnson2018image} and \citep{xu2017attngan} as can be seen in Figure \ref{fig:comparison}. The scene graph in the first step contains two objects and the relationships between them. An additional object and its relationship with other objects is added to the scene graph at each of the next two steps. Note that the two baselines do not generate incrementally but for fair comparison, we generate outputs from them by feeding different amounts of information (scene graph or text) in three independent forward passes.

As can be seen, the first baseline \cite{johnson2018image} is able to capture the semantic context provided by the graph. However (i) it fails to preserve consistency over multiple passes and generates a completely new image for each scene graph, agnostic of what it had generated at the previous step and (ii) the images generate are of poor quality. The second baseline \citep{xu2017attngan} produces visually pleasing and high resolution images but completely fails to capture any semantic context provided from the graph. Our model, on the other hand, is capable of incrementally adding new objects to the image created in the previous step in accordance with the relationships defined in the scene graph. Additionally, the quality of generated images is significantly improved, since at each step the model has to generate only a few objects rather than generating cluttered scenes with multiple objects, hence enabling it to better generate scene semantics.



We present comprehensive results generated by our model in Figure \ref{fig:sample_outputs}. It can be seen in Figures 4(c,f,h) that the model starts by generating objects as described by the scene graph and outputs noise in the background when it does not have enough information provided as input. As the background information is added in the scene graph, background objects like grass and sky begin to materialize. However it can also be seen that sometimes due to inherent biases in the dataset, the model begins to hallucinate the background even when no information is provided explicitly. In Figure 4(a), even though there is no mention of rock or water in the initial graph, the model is hallucinating objects of similar shapes at similar locations.

\subsection{Quantitative Evaluation}

We use Inception Score \citep{salimans2016improved} for evaluating the quality of the images generated from our models. Inception Score uses an ImageNet based classifier to provide a quantitative evaluation of how realistic generated images appear. Inception Scores were originally proposed with the two main goal. Firstly, the images generated should contain clear objects (i.e.
the images are sharp rather than blurry), (or, for image $x$ and label $y$, $p(y|x)$
should be low entropy). 
%In other words, the Inception
%Network should be highly confident there is a single
%object in the image. 
Secondly,  the generative algorithm should output a high diversity
of images from all the different classes in ImageNet,
or $p(y)$ should be high entropy.

\begin{table}[h]
    \centering
        
    \begin{small}
    \begin{tabular}{lcccc}
        \toprule
        Ground Truth & \citet{johnson2018image} & Step 1 (Ours) & Step 2 (Ours) & Step 3 (Ours) \\
        \midrule
        % Validation Accuracy ($\%$) & 75.59 & \textbf{82.70} & 77.99\\
        6.13         & 3.05  & \textbf{3.68}   & \textbf{5.02}   & \textbf{4.14} \\
        \bottomrule
    \end{tabular}
    \end{small}
    \caption{Inception Scores for Ground Truth Images, images generated from Sg2im and the three steps from our model}
    \label{tab:inception}
\end{table}


The inception scores are reported in Table \ref{tab:inception}. We compare the inception score of the images generated from the baseline model sg2im with the full scene graph of the ground truth images. For our sequential generation model, we report the scores over three steps of generation, where at the third step the scene graph is the full scene graph corresponding to the ground truth image. We observe that due to our modified loss formulation and incremental generation, our model performs better in inception scores in all three steps.
%We also note that Stage 2 performs the best. 
%From our observations this is because the vividness of the image colors and object definitions is the best at the stage 1, and begin to fade out stage 2 onwards. \\

Next, we evaluate how well our model retains the generated image from the previous step when adding in information to the image in the subsequent step (i.e., how ``visually consistent'' the generated images are). We use the perceptual similarity loss proposed by \cite{zhang2018perceptual}, and report the mean losses in Table \ref{tab:percep}. As seen both in the table and qualitatively in Figure \ref{fig:comparison}, our model is much more successful at preserving context and previously generated content over subsequent steps. 






\begin{table}[h]
    \centering
        
    \begin{small}
    \begin{tabular}{lcccc}
        \toprule
        Method & Step 1 to Step 2 & Step 2 to Step 3 \\
        \midrule
        % Validation Accuracy ($\%$) & 75.59 & \textbf{82.70} & 77.99\\
        \citet{johnson2018image}         & 0.658  & 0.496   \\
        Ours  & \textbf{0.477} & \textbf{0.421}\\
        \bottomrule
    \end{tabular}
    \end{small}
\caption{Mean Perceptual similarity loss, evaluated between the images generated images of sg2im and our proposed model. Lower is better.}
    \label{tab:percep}
\end{table}


\begin{comment}

\subsection{AttnGan}
% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.5\linewidth]{images/attn_results_1.png}
% \end{center}
%   \caption{(a) shows a sample result of AttnGAN where only a where abstract notion of the text description is captured with no clear resemblance of objects. (b) shows a sample result of AttnGAN where although the image is of a high quality, the semantics of the text description are completely lost in the generation.}
% \label{fig:attn_results1}
% \end{figure}

% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.5\linewidth]{images/attn_results_2.png}
% \end{center}
%   \caption{Comparison of two sample generations from AttnGAN differing only in the presence of adjective in the text description used. Here, we can see that although `well-lit' is used as an adjective in (a), (b) seems more well-lit based on the generation.}
% \label{fig:attn_results2}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/attn_results_comb.png}
    \caption{(a) shows a sample result of AttnGAN where only a where abstract notion of the text description is captured with no clear resemblance of objects. (b) shows a sample result of AttnGAN where although the image is of a high quality, the semantics of the text description are completely lost in the generation. Comparison of two sample generations from AttnGAN differing only in the presence of adjective in the text description used. Here, we can see that although `well-lit' is used as an adjective in (c), (d) seems more well-lit based on the generation.}
    \label{fig:attn_results1}
\end{figure}
Although \cite{xu2017attngan} show results for multiple datasets, we obtained results only for MS-COCO dataset for our first baseline since we will be using that for our task of incremental image generation. The results are shown in Figure \ref{fig:attn_results1}. As can be seen from the results, AttnGan has many issues. Although it produces high resolution images, it only captures an abstract notion of the description represented by the text and does not preserve the saliency of objects. We can see in Figure \ref{fig:attn_results1}a that although the background of the image is that of water, we do not get any clear picture of the girl surfing, as is expected by the text. Moreover, AttnGan fails to preserve text semantics and although it is somewhat able to generate the individual objects mentioned in the text, it is not able to accurately display the relationship between them. For example, In Figure \ref{fig:attn_results1}b, we can see an abstract image of a girl and a pizza, but it is unclear as to who is eating what. Additionally, we observed that there is a heavy bias in the dataset, such that changing adjectives describing the objects in the description do not produce any changes in the generated images. In Figure \ref{fig:attn_results1}d, we can see that removing the adjective 'well lit' which describes the skyscrapers, did not result in an image with a dark skyscraper. Hence, the model did not really take into account the adjective 'well lit' while it was generating the first image in Figure \ref{fig:attn_results1}c. It just generated a well lit skyscraper by taking into account the inherent bias present in the dataset. Lastly, we also observed that AttnGan can neither handle multiple objects in the description nor can it handle an incremental addition of objects. As we can see in Figure \ref{fig:attn_results3} (Appendix), we changed the description slightly by adding 'floating on top of a lake', but we do not see any lake added in the image. Moreover, it resulted in the distortion of the image generated by the original description as even the fruits in original image are not clearly visible anymore.  

\subsection{Image Generation using Scene Graphs}

\begin{figure}[h]
\begin{center}
\includegraphics[width=1\linewidth]{images/sg2im_results_2.png}
\end{center}
   \caption{Sample images generated using \cite{johnson2018image}. Here we fed incrementally growing scene graphs to the model and generate a sequence of images. As can be seen, the scene graphs for each generated image in shown below the corresponding image. The blue boxes denote the relationships between different object/stuff entities denoted by red boxes. By generating a sequence of images, we can clearly observe that there is no consistency between the incremental images generated. This clearly highlights the shortcoming of the approach that is the inability to generate images with growing scene graphs maintaining the consistency.}
\label{fig:sg2im_results1}
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.3\linewidth]{images/sg2im_results_3.png}
\end{center}
   \caption{Sample images generated using \cite{johnson2018image} where we used the same set of object/stuff entities organized as two different scene graphs having different relationships. Clearly, there is no perceptible distinction between the two image generated which shows that the training is highly biases towards the objects and not the relationships.}
\label{fig:sg2im_results2}
\end{figure}

For our second baseline, we obtained the results from \cite{johnson2018image} which are shown in Figures \ref{fig:sg2im_results1}, \ref{fig:sg2im_results2} and \ref{fig:sg2im_results3}. 

Scene graphs are a powerful structured representation
for both images and language, and they describe the objects and relationships between these objects.  A scene graph is a tuple (O, E) where O is the set of objects and E is a set of directed edges. In each of the shown results, we include the scene graph representation used to generate the image below the corresponding image. The blue boxes denote the relationships between different object/stuff entities denoted by red boxes.

From all the sample generations, we can clearly observe that there is no consistency between images corresponding to incrementally growing scene graphs. In Figure \ref{fig:sg2im_results1} and \ref{fig:sg2im_results2}, we show a sequence of generated images where we incrementally add new entities to the scene graphs. We can observe that all the images are quite different from each other perceptually. Clearly, the method lacks a mechanism to generate images with incrementally growing scene graphs.

Another major limitation of this model is that it overfits to the input graph. There is no variation observed by running the model multiple times with the same input graph. Moreover the model also overfits to the objects in the input scene graph. As can be seen in Figure \ref{fig:sg2im_results2}, even if we change the relationship of the object `tent' with respect to the other objects, the same image is generated. Furthermore, the model completely ignores generating uncommon objects that it encounters. As we can see in Figure \ref{fig:sg2im_results2}, the model has completely foregone the generation of the `tent' even though it is mentioned in both the scene graphs. 

Additionally, as can be observed in all Figures, the model produces low resolution poor quality images at the expense of maintaining the semantics of the text description. Although the model tries to preserve saliency and object relationships, it causes photo-realism to suffer. As we can see in Figure \ref{fig:attn_results1}, the model tries to generate an additional bear to left of the original bear when we add it into the scene graph, the image of the bear is not really recognizable and it could be interpreted as a gorilla or as an elephant by a person who hasn't seen the descriptions. Lastly, we can observe in Figure \ref{fig:sg2im_results3} (Appendix) that the quality of objects classes is poorer than stuff classes. We can see that while the model generates relatively convincing images of stuff classes like grass, sky and mountains, the object classes like sheep and horse are much worse in quality. 

\end{comment}


% \subsection{Qualitative results of image quality enhancement}
% We visualize the results of our StackGAN based image quaity enhancement in Fig. \ref{fig:stackgan_results}. We observe a considerable improvement in image quality with our StackGAN based refinement network approach. For would like to note that for training this in parallel, we used the images generated by our baseline, sg2im, as the coarse 64x64 input. We expect an even further quality improvement by retraining using the images generated by our model.


% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=\linewidth]{images/stackgan_results.png}
% \end{center}
%   \caption{Sample images generated using our StackGAN based refinement network proposed in Section 3.3. Top row: 64x64 images generated from sg2im, our baseline model. Middle row: 256x256 outputs generated by our StackGAN based enhancement. Bottom row: Ground truth images in MS COCO}
% \label{fig:stackgan_results}
% \end{figure}




==> Multimodal - ICLR 2019-new-2/intro.tex <==
\section{Introduction}
To truly understand the visual world, our models should be able to not only recognize images but also generate them. Generative Adversarial Networks, proposed by \citet{goodfellow2014generative} have proven immensely useful in generating real world images. GANs are composed of a generator and a discriminator that are trained with competing goals. The generator is trained to generate samples towards the true data distribution to fool the discriminator, while the discriminator is optimized to distinguish between real samples from the true data distribution and fake samples produced by the generator.
The next step in this area is to generate customized images and videos in response to the individual tastes of a user. A grounding of language semantics in the context of visual modality has wide-reaching impacts in the fields of Robotics, AI, Design and image retrieval. To this end, there has been exciting recent progress on generating images from natural language descriptions. Conditioned on given text descriptions, conditional-GANs \citep{reed2016generative} are able to generate images that are highly related to the text meanings. Samples generated by existing text-to-image approaches can roughly reflect the meaning of the given descriptions, but they fail to contain necessary details and vivid object parts.

Leading methods for generating images from sentences struggle with complex sentences containing many objects.  A recent development in this field has been to represent the information
conveyed by a complex sentence more explicitly as a scene graph of objects and their relationships \citep{johnson2018image}. Scene graphs are a powerful structured representation for both images and language; they have been used for semantic image retrieval \citep{johnson2015image} and for evaluating \citep{anderson2016spice} and improving \citep{liu2017improved} image captioning. In our work, we propose to leverage these scene graphs by incrementally expanding them into more complex structures and generating corresponding images. Most of the current approaches lack the ability to generate images incrementally in multiple steps while preserving the contents of the image generated so far. We overcome this shortcoming by conditioning the image generation process over the cumulative image generated over the previous steps and over the unseen parts of the scene graph. This allows our approach to generate high quality complex real-world scenes with several objects by distributing the image generation over multiple steps without losing the context. Recently, \citet{elkeep} proposed an approach for incremental image generation but their method is limited to synthetic images due to the need of supervision in the intermediate step. Our approach circumvents the need for intermediate supervision by enforcing perceptual regularization and is therefore compatible with training for even real world images (as we show later). 

A visualization of our framework's outputs with a progressively growing scene graph can be seen in Figure \ref{fig:cover}. We can see how at each step new objects get inserted into the image generated so far without losing the context.  
To summarize, we make the following contributions,
\begin{itemize}
    \item We present a framework to generate images from structured scene graphs that allows the images to be interactively modified, while preserving the context and contents of the image generated over previous steps.
    \item Our method does not need any kind of intermediate supervision and hence, is not limited to synthetic images (where you can manually generate ground truth intermediate images). It is therefore useful for generating real-world images (such as for MS-COCO) which, to the best of our knowledge, is the first attempt of its kind.
\end{itemize}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Related Work}
% \textbf{Image generation from text.}
Generating images from text descriptions is of great interest, both from a computer vision perspective, and a broader artificial intelligence perspective.
Since the advent of Generative Adversarial Networks (GANs), there have been many efforts in this direction \citep{huang2018introduction}. 
\citet{ouyang2018generating} proposed a framework based on an LSTM and a conditional GAN to incrementally generate an image using a sentence. The words in the sentence were encoded using word2vec, and passed through an LSTM. A skip-though
vector representing the semantic meaning of an entire sentence is used as the conditioning for the GAN.
However, all of these works mostly focus on generating images with single objects (such as faces or flowers or birds). Even within these objects, the avenues of variance is quite limited. 
Generating more complex scenes with multiple objects and specific relationships between those objects is an even harder research problem.

\citet{zhang2017stackgan} proposed an architecture based on multiple GANs stacked together, generating images in a coarse-to-fine manner. They later also proposed arranging the generators in a tree-like structure for improved results \citep{zhang2017stackgan++}. More recently, \citet{hong2018inferring} proposed an end-to-end pipeline for inferring scene structure and generating images based on text descriptions. A similar approach was taken by \citet{tan2018text2scene}, where they used attention-based object and attribute decoders to infer bounding box locations of  objects in the scene. However, for images with several objects such as in COCO-Stuff, the captions are often not descriptive enough to capture all the objects. Furthermore, the captions don't describe the relations between the objects in the image effectively. AttnGANs also begin with a low-resolution image, and then improve it over multiple steps to come up with a final image. However, there's no mechanism to capture consistency during incremental image generation. A more detailed failure case analysis is done in Section~\ref{experiments}.

Most recently, \citet{johnson2018image} proposed to use scene-graphs as a convenient intermediate for image synthesis. Scene-graphs provide an efficient and interpretable representation of the objects in an image and their relationships. The input scene graph is processed with a graph convolution network which passes information along edges to compute embedding vectors for all objects. These vectors are used to predict bounding boxes and segmentation masks for all objects, which are combined to form a coarse scene layout. The layout is passed to a cascaded refinement network which generates an output image at increasing spatial scales. The model is trained adversarially against a pair of discriminator networks which ensure that output images look realistic.
However, this model does not account for object saliency or temporal consistency in the generated images. It also fails for highly complex scene where there are several objects due to a single-pass image generation. A more detailed failure case analysis is done in Section \ref{experiments}.

Another recent work by \citet{elkeep} introduces a conditional text-to-image based generation approach to generate images iteratively, keeping track of ongoing context and history. Their method uses GRU to process text instructions into embeddings which go through conditioning augmentation and are fed into a GAN to generate contents on a canvas. They use a convex combination of feature maps to ensure consistency. Due to the availability of structured information in the form of scene graphs, we can instead filter out the latent embeddings of the already generated objects, thus allowing for better textural consistency. Moreover, their approach suffers from the drawback of needing supervision at every stage of generation for training and is therefore limited to only synthetic scenarios (such as CoDraw and i-CLEVR where intermediate images can be easily rendered). On the contrary, our approach employs perceptual similarity based regularization and effective use of graph-based embeddings to circumvent the need of ground truth for intermediate steps, making it compatible with even real-world images. 

% \paragraph{Image modification.}
% One of the major avenues in research in computer vision has been the task of "inpainting", i.e. filling in a missing region in an image. Earlier approaches relied on finding nearest-neighbour matches within the image or in a dataset to complete missing regions. More recently, works such as \cite{yeh2017semantic,iizuka2017globally} have used architectures such as fully convolutional nets or GANs, coupled with discriminators, to complete images.
% \cite{shetty2018adversarial} proposed a GAN based framework for removing objects in an image by generating a mask and inpainting the masked area. They used a combination of 3 adversarial losses based on object classification and image and mask realism.

% \paragraph{Text to Scene graph.} It is also of great research interest to be able obtain precise scene graphs from detailed text descriptions of an image. Earlier works \cite{coyne2001wordseye} have proposed parsing the dependency structure of detailed text descriptions and converting them into query formats for a 3D cad model database. More recently, \cite{schuster2015generating} proposed rule-based and classifier-based parsers for obtaining such graphs from descriptions.

==> Multimodal - ICLR 2019-new-2/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Multimodal - ICLR 2019-new-2/method.tex <==
\section{Method}

As in most modern conditional image-generation formulations, we follow a generative-adversarial approach to image generation. Here the adversarial network penalizes the network based on how realistic the generated images are, as well as whether the required objects are present in them. Furthermore, a key part of the task is to preserve the relations between objects as specified in the scene graph in the generated image as well. 

\begin{figure*}[t!]
\begin{center}
\includegraphics[width=\linewidth]{images/architecture_2.png}
\end{center}
    \caption{Model architecture for incremental image generation using scene graphs. The Graph Convolution Network takes as input the scene graph and produces object embeddings which are then fed to the Scene Layout Network. The SLN generates a layout by predicting the bounding boxes and segmentation masks for the objects. These are finally sent to the Cascaded Refinement Network which generates the image corresponding to the graph. This process is called iteratively to add objects in the image.}
\label{fig:archi}
\end{figure*}
\subsection{Image generation from scene graphs}
For our baseline approach for generating images from scene graphs, we adopt the architecture proposed by \cite{johnson2018image}. The architecture consists of 3 main modules, a Graph Convolution network (GCN), Layout Prediction Network (LN) and a Cascade Refinement Network (CRN), which we describe in more detail below. For brevity, we omit an exhaustive background description of these modules and request the reader to refer to the original paper for further details. Figure~\ref{fig:archi} provides an overview of the full model architecture.

\textbf{Graph Convolution Network.} The Graph Convolution Network (GCN) is composed of several graph convolution layers, and can operate natively on graphs. GCN takes an input graph and computes new vectors for each node and edge. Each graph convolution layer propagates information along edges
of the graph. The same function is applied to all graph edges, which ensures that a single convolution layer can work with arbitrary shaped graphs. 

\textbf{Layout Prediction Network.} The GCN outputs an embedding vector for each object. These object embedding vectors are used by the layout prediction network to compute a scene layout by predicting a segmentation mask and bounding box for each object. Mask regression network and a box regression network are used to predict a soft binary mask and a bounding box, respectively. The layout prediction network hence acts as an intermediary between the graph and image domains. 

\textbf{Cascade Refinement Network.} Given a scene layout, the Cascade Refinement Network (CRN) is responsible for generating an image which respects the object positions in the scene layout. The CRN consists of a series of convolutional refinement modules. The spatial resolution doubles between modules; which ensures that image generation is happening in a coarse-to-fine manner. The scene layout is first downsampled to the module input resolution and then fed to the module along with the previous module's output. Both these inputs are concatenated channel-wise and then passed to a pair of $3 \times 3$ convolution layers. This output is upsampled using nearest-neighbor
interpolation and then passed to the next module. The output from the last module is finally passed to 2 convolution layers to produce the output image.  

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.7\textwidth]{images/comparison_2.png}
%     \caption{Comparison of our results with baseline approaches--sg2im and AttnGAN. While sg2im captures the scene graph's semantic context, it lacks consistency over multiple passes and the generated images are of poor quality. AttnGAN on the other hand generates higher resolution images but doesn't capture semantic context from the scene graph. Our model addresses both of these shortcomings by incrementally adding objects in accordance with the scene graph and  generating higher quality images.  }
%     \label{fig:comparison}
% \end{figure*}


\subsection{Sequential generation of images with context preservation}
Our method allows for preserving context across the sequentially generated images by conditioning subsequent steps of image generation over certain information from previous steps.

\begin{itemize}
    \item We extend \cite{johnson2018image} with a recurrent architecture that generates images using incrementally growing scene graphs using the components discussed in previous section as shown in Figure~\ref{fig:archi}.
    \item To ensure that the image generated in the current step preserves the visual context from the previous steps, we replace three channels of the noise passed to CRN with the RGB channels of the image generated in the previous step. This encourages the CRN to generate the new image as similar as possible to the previously generated image.
    \item Moreover, we want the SLN to generate a layout corresponding to only the newly added objects in the scene graph. To this end, we remove the representations generated by GCN corresponding to the objects generated in previous steps.
    \item We do not have any ground truth for the intermediate generated images so we use perceptual loss for images generated in the intermediate steps to enforce the images to be perceptually similar to the ground truth final image. We do have L1 loss between the final image generated and the ground truth.
\end{itemize}
Concretely, we train the network with the following losses:
\begin{enumerate}
    \item Adversarial losses: We use an image level and an object level discriminator to ensure realism of the images and presence of the objects. These are trained as in the regular GAN formulation : 
    $\mathcal{L}_{GAN} = E_{x \sim p_{real}} log D(x) + E_{x\sim p_{fake}} log(1-D(x))$
    \item Box loss: Penalizes L1 distance between ground truth boxes from MS COCO vs the predicted labels as $\mathcal{L}_{box} = \sum_i^n ||b-b'||$  
    \item Mask loss: Penalizes difference between the masks predicted vs the ground truth masks, using cross entropy loss.
    
    \item L1 pixel loss: Penalizes the difference between the ground truth image from MS COCO and the final generated image at the end of the incremental generation. L1 pixel losses are also used to penalize the difference  between the previous and current generated image. $\mathcal{L}_{pixel} = ||I_G-I_{final}||$
    
    \item Perceptual Similarity Loss: Serves as a regularization to ensure that the images generated at different steps are contextually similar to each other. Since we do not have ground truth for intermediate steps, we introduce an additional perceptual similarity loss using \citet{zhang2018perceptual} between the final ground truth image and the different images generated in the intermediate steps. This allows the model to `hallucinate' for the intermediate steps in a way that the contents of the image are similar to the ground truth. $\mathcal{L}_{perceptual} = ||P^{\phi}(I_k) - P^{\phi}(I_G) ||^2$ where $P^{\phi}$ is the function computing a latent embedding that captures the perceptual characteristics of an image.
\end{enumerate}
  Thus we can provide additional supervision on the coordinates of the bounding boxes predicted by the layout network, to explicitly ensure the relations are preserved. 


% \subsection{Image quality enhancement}

% We also focus on improving the quality of the images generated by the baseline model. By default, the images are generated at a 64x64 resolution. We later show in our experiments that our recurrent network and modifications to the loss terms by itself lead to improvements in the image quality. However, we further seek to enhance the generated images by drawing on insights drawn from StackGAN \cite{zhang2017stackgan}. The authors if StackGAN proposed a two-stage coarse-to-fine generation framework that generated an image conditioned on a text embedding. They proposed a conditioning augmentation, which augmented the size of the training data and lead to a smoother manifold of the GANs.
% For our purposes, we remove the first stage of the StackGAN, instead using the 64x64 image generated by our network, as the input to the second stage. For the conditioning, we use the layout matrix generated by the LN, with the same conditioning augmentation applied. We skip the spatial replication as the Layout already has spatial info and is of the same dimensions as the image. The output of the generator is a higher resolution 256x256 image.

% \begin{figure*}[h]
% \begin{center}
% \includegraphics[width=\linewidth]{images/StackGAN.png}
% \end{center}
%     \caption{Our proposed architecture for image quality enhancement based on \cite{zhang2017stackgan}. The 64x64 image generated by the main architecture is concatenated with a conditioning augmented layout map generated by the SLN. This is fed to the upsampling generator, which generates a 256x256 output. The images are sent to the discriminator along with the layout embedding. }
% \label{fig:stackgan}
% \end{figure*}


% \section{Baseline Models}
% \subsection{AttnGAN}

% The Attentional Generative Adversarial Network (or AttnGAN) begins with a crude, low-resolution image, and then improves it over multiple steps to come up with a final image. AttnGAN starts off by generating an image from (random noise + a summation of the caption’s token-embeddings).

% However, one of the issues with generating an image from a combined sentence vector, is that we lose a lot of the fine-grained details hidden in individual words. To remedy this, AttnGAN uses a combination of Attention and GAN at every stage, to iteratively add details to the image.

% After the concept of multi-stage image refinement, the second key feature of this framework is The Deep Attentional Multimodal Similarity Model (DAMSM). DAMSM takes as input an image and the caption, and provides feedback on how well the two fit together. It does this as follows:
% \begin{enumerate}
%     \item Using a standard CNN, the image is converted into a set of feature maps. Each feature map essentially signifies some concept/sub-region in the image.
%     \item The dimensionality of the feature maps is made equal to that of the word embeddings, so that they can be treated as equivalent entities.
%     \item Based on each token in the caption, attention is applied over the feature maps, to compute a weighted average of them. This attention-vector essentially represents the image’s abstraction of the token.
%     \item Finally, DAMSM is trained to minimize the difference between the above attention-vector (visual portrayal of the word) and the word-embedding (textual meaning of the word).
% \end{enumerate}





% % \begin{figure}[h]
% % \centering
% % \includegraphics[width=0.9\linewidth]{images/AttnGAN.png}


% % \caption{AttnGAN Model Architecture}
% % \label{fig:AttnGAN}
% % \end{figure}

% \subsection{Image generation using scene graph}

% \begin{figure*}
% \begin{center}
% \includegraphics[width=1\linewidth]{johnson.png}
% \end{center}
%   \caption{The architecture proposed in \cite{johnson2018image} for generation of complex scenes from scene graphs. Input scene graph is processed by a Graph Convolutional Network (GCN) to output object based embeddings. Based on these embeddings, the network predicts bounding boxes and segmentation mask which are translated by a Cascade Refinement Network to generate the final image.}
% \label{fig:arch}
% \end{figure*}

% This paper proposes a method for generating images from text-based scene graphs, enabling explicitly reasoning about objects and their relationships.

% The model \ref{fig:arch} uses graph convolution to process input graphs, computes a scene layout by predicting bounding boxes and segmentation masks for objects, and converts the layout to an image with a cascaded refinement network. The network is trained adversarially against a pair of discriminators to ensure realistic outputs.

% This approach is validated  on Visual Genome and COCO-Stuff, where qualitative results, ablations, and user studies demonstrate our method's ability to generate complex images with multiple objects.
